Accelerated Distributed Stochastic Non-Convex Optimization over Time-Varying Directed Networks

Distributed stochastic non-convex optimization problems have recently received attention due to the growing interest of signal processing, computer vision, and natural language processing communities in applications deployed over distributed learning systems (e.g., federated learning). We study the setting where the data is distributed across the nodes of a time-varying directed network, a topology suitable for modeling dynamic networks experiencing communication delays and straggler effects. The network nodes, which can access only their local objectives and query a stochastic first-order oracle to obtain gradient estimates, collaborate to minimize a global objective function by exchanging messages with their neighbors. We propose an algorithm, novel to this setting, that leverages stochastic gradient descent with momentum and gradient tracking to solve distributed non-convex optimization problems over time-varying networks. To analyze the algorithm, we tackle the challenges that arise when analyzing dynamic network systems which communicate gradient acceleration components. We prove that the algorithm's oracle complexity is $\mathcal{O}(1/\epsilon^{1.5})$, and that under Polyak-$\L$ojasiewicz condition the algorithm converges linearly to a steady error state. The proposed scheme is tested on several learning tasks: a non-convex logistic regression experiment on the MNIST dataset, an image classification task on the CIFAR-10 dataset, and an NLP classification test on the IMDB dataset. We further present numerical simulations with an objective that satisfies the PL condition. The results demonstrate superior performance of the proposed framework compared to the existing related methods.

==> n_algorithm.tex <==

%We start this section by formalizing the problem of distributed non-convex optimization under the stochastic first-order oracle.

%\subsection{Learning task}

Assume that $n$ nodes are collaboratively solving the decentralized non-convex optimization problem \eqref{eq:prob} while communicating over a time-varying directed network.
% \begin{equation} \label{eq:prob}
% \min_{\mathrm{\mathbf{x} \in \mathbb{R}^d}} \left[f(\mathbf{x}):=\frac{1}{n}\sum_{i=1}^n f_i(\mathbf{x})\right],
% \end{equation}
% where $f_i(\mathbf{x}): \mathbb{R}^d \to \mathbb{R}$ for $i \in [n]:=\left\{1, ..., n \right\}$ denotes the non-convex objective function locally minimized at node $i$; in machine learning context, this describes the setting where each node trains a local model by optimizing a cost function with $d$ parameters, and collaborates with other nodes to find the global model. The local objectives satisfy the smoothness condition (see Assumption \ref{assumption1} below). The nodes can communicate information over a directed network. 
Each node $i$ in the network trains a local model and computes a sequence of local model estimates $\{\x_t^i \}$ towards a first-order stationary point of the global objective $f$, starting from a pre-specified initialization point $\x_0^i$. To update its local model estimate, node $i$ accesses a random local data point $ \mathbf{\xi}^i_{t} $ and queries the stochastic first-order oracle for a stochastic gradient, $\nabla f_i(\mathbf{x}, \mathbf{\xi}^i_{t} )$, given the input $\x$. To characterize the sequence of random local data points, we consider the filtration induced by the data points of all nodes in the network,
\begin{equation}
\begin{aligned}
    \mathcal{F}_0  = \{\Omega, \phi \},\;\;
    \mathcal{F}_t  = \sigma(\{\mathbf{\xi}^i_{0}, \mathbf{\xi}^i_{1}, \cdots, \mathbf{\xi}^i_{t-1}, i \in \mathcal{V} \}), \forall t \geq 1,
\end{aligned}
\end{equation}
where $\phi$ is the empty set and $\{\mathcal{F}_t\}$ is an increasing family of $\sigma$-algebras. The input vector $\x$ at iteration $t$ is $\mathcal{F}_t$-measurable. We denote the probability space by $\{\Omega, \mathbb{P}, \mathcal{F} \}$. We make the following assumptions on the stochastic first-order oracles, the global objective, and the communication network.

\begin{assumption}\label{assumption1}
For all $i \in \mathcal{V}$ and all $t \geq 0$, we assume:
1.~Unbiasedness of the conditional expectation
    \begin{align*}
        \mathbb{E}[\nabla f_i(\mathbf{x}, \mathbf{\xi}^i_{t} ) |\mathcal{F}_t ] = \nabla f_i(\x).
    \end{align*}
2.~Bounded variance of the estimated gradient,
    \begin{align*}
        \mathbb{E}\|\nabla f_i(\mathbf{x}, \mathbf{\xi}^i_{t} ) - \nabla f_i(x) \|^2 \leq \nu_i^2.
    \end{align*}
It will be convenient to introduce $\Bar{\nu}^2 = \frac{1}{n}\sum_{i=1}^n \nu_i^2$.\\
3.~Independent random selection, i.e., the random vectors $\{\mathbf{\xi}^i_{0}, \mathbf{\xi}^i_{1}, \cdots, \mathbf{\xi}^i_{t-1}\}$, $i \in \mathcal{V}$, are independent.\\
4.~The mean-squared smoothness,
    \begin{align*}
        \mathbb{E}\|\nabla f_i(\mathbf{x}, \mathbf{\xi}^i_{t} ) - \nabla f_i(\mathbf{y}, \mathbf{\xi}^i_{t} ) \|^2 \leq L^2 \mathbb{E}\|\x - \mathbf{y} \|^2.
    \end{align*}
%\end{enumerate}
\end{assumption}
The first three assumptions are widely used in the analysis of stochastic first-order optimization algorithms \cite{bottou2010large}. The last assumption requires the $L$-smoothness of the stochastic gradient on average with respect to any two inputs. The mean-squared smoothness further implies the smoothness of each local objective $f_i$, and consequently implies the $L$-smoothness of the global objective \cite{fang2018spider,arjevani2019lower}. 

\begin{assumption}\label{assumption2}
The global objective is lower bounded, 
\begin{equation*}
    f^* = \inf_{\x } f(\x) > -\infty.
\end{equation*}
\end{assumption}

\begin{assumption}\label{assumption3}
The network is directed and time-varying. At time $t$, the network is strongly-connected with a column stochastic weight matrix $W_m^{(t)}$. 
\end{assumption}

The above assumption on network topology is standard in distributed optimization \cite{nedic2017achieving} and more general than the static network assumption in \cite{assran2019stochastic}. Elaborating on Assumption~3, let us consider the mixing matrix $W_m^{(t)} := [w_{ij}^{(t)}]$ which captures properties of the communication links in the network;
%Specifically, it holds that $w_{ij}^{(t)}>0 $ if and only if $ (i, j) \in \E(t)$ or $i = j$.
$w_{ij}^{(t)} = \frac{1}{d_j^{out, t}+1}>0 $ if and only if $ (i, j) \in \E(t)$ or $i = j$, where $d_j^{out, t} $ is the out-degree of agent $j$ at time $t$.We assum e that node $i$ knows the nodes it receives messages from and sends messages to, i.e., the $i$-th row and column of $W_m^{(t)}$ are known to node $i$. The column stochastic mixing matrix $W_m^{(t)}$ has the left eigenvector $\mathbf{1}_n$ and a positive right eigenvector $\pi$, i.e., $\mathbf{1}_n^\top W_m^{(t)} = \mathbf{1}_n^\top $ and $W_m^{(t)}\pi = \pi$. %According to the Perron-Frobenius theorem,  {\color{black}{the limit of the powers of the mixing matrix over a time duration $t$, $W_m^t $, }} satisfies $W_m^{\infty} = \lim_{t \to \infty}W_m^t = \pi \mathbf{1}_n^\top$. 

%Using the weighted Euclidean norm defined in Section \ref{sec:notation}, one obtains that the spectral gap $1 - \lambda$ for the mixing matrix $W_m$ satisfies
%   $0 < 1- \lambda < 1.$

% Furthermore, it is readily verified that the weighted norm follows $\| \cdot \|_{\pi} \leq \sqrt{ \barbelow{\pi}} \| \cdot \|_2 $ and $\| \cdot \|_2 \leq \sqrt{\bar{\pi}} \| \cdot \|_{\pi}$, where $\barbelow{\pi} $ and $ \bar{\pi}$ represent the maximum and minimum element of the vector $\pi$, respectively. 

\vspace{-2mm}

\section{The Push-ASGD Algorithm}
\setlength{\intextsep}{0pt}
\definecolor{light-gray}{gray}{0.9}
\begin{algorithm}[t]
\caption{Push Accelerated Stochastic Gradient Descent Algorithm (Push-ASGD)}
\begin{algorithmic}[1]
   \STATE {\bfseries Input:} Initialize values $\mathbf{x}^i_0 = \Bar{\mathbf{x}}_0$; $y_0^i = 1$ ; $\mathbf{z}^i_0 = \mathbf{x}^i_0 $; step size $\alpha$; $\beta \in (0, 1)$; time-varying column-stochastic mixing matrix $W_m^{(t)} := [w^{(t)}_{ij}]$; $T \in \mathbf{Z}^+$\;
\STATE Sample $\{ \mathbf{\xi}_{0, r}^i\}_{r=1}^b$ and initialize the gradient $\mathbf{g}_0^i = \frac{1}{b} \sum_{r=1}^b\nabla f_i(\mathbf{z}^i_0, \mathbf{\xi}_{0, r}^i)$ and the gradient estimator $\mathbf{v}^i_{0} = \mathbf{g}_0^i$; \;
   \FOR{$t=1$ {\bfseries to} $T-1$}
   \STATE Update the local estimate of the solution
   
   \colorbox{light-gray}{$\mathbf{x}_{t+1}^i = \sum_{j=1}^n w^{(t)}_{ij}(\mathbf{x}_t^j - \alpha \mathbf{g}_{t}^j) $}
   \STATE Update auxiliary variables
   
    \colorbox{light-gray}{$y_{t+1}^i = \sum_{j=1}^n w^{(t)}_{ij}y_t^j , \ \mathbf{z}_{t+1}^i =\frac{ \mathbf{x}_{t+1}^i} { y_{t+1}^i }$} 
    \STATE
    Sample $\mathbf{\xi}_t^i$ and update the local stochastic gradient estimator
    
    \colorbox{light-gray}{$ \mathbf{v}^i_{t+1} =  \nabla f_i(\mathbf{z}^i_{t+1}, \mathbf{\xi}^i_{t}) + (1-\beta)(\mathbf{v}^i_{t} -\nabla f_i(\mathbf{z}^i_{t}, \mathbf{\xi}^i_{t} ) ) $} \;
    \STATE
    Update the gradient tracker 
    
    \colorbox{light-gray}{$ \mathbf{g}_{t+1}^i = \sum_{j=1}^n w^{(t)}_{ij}(\mathbf{g}_t^j + \mathbf{v}_{t+1}^j - \mathbf{v}_{t}^j ) $} \;
   \ENDFOR
\end{algorithmic}
\label{non_cvx_algorithm}
\end{algorithm}

In this section we present an algorithm for distributed non-convex optimization over directed time-varying networks. At a high level, the algorithm relies on the push-sum protocol \cite{kempe2003gossip} to perform average consensus, and deploys stochastic gradient estimator of the unknown global gradient while simultaneously reducing the variance/noise in the local updates via momentum.

At iteration $t$, node $i$ updates its local model $\x^i_t$ by fusing the messages $\mathbf{x}_t^j$ received from its neighbors according to%the  descent operation,
\begin{equation}
    \mathbf{x}_{t+1}^i = \sum_{j=1}^n w_{ij}^{(t)}(\mathbf{x}_t^j - \alpha \mathbf{g}_{t}^j),
\end{equation}
where $\mathbf{g}_{t}^j$ denotes the local stochastic gradient estimate, specified below.

Since $W_m$ is column-stochastic, {\color{black}{the powers of $W_m$ over a time duration $t$, $W_m^t $,}} generally differ from $\frac{ \mathbf{1} \mathbf{1}^T}{n}$, biasing each node to a different model. Therefore, following  \cite{nedic2016stochastic}, for each node $i$ with the local model $\x^i_t$ at time $t$, we introduce an auxiliary scalar $y^i_t$ and compute a recovering model $\z^i_t = \x^i_t / y^i_t$ to enable de-biasing the local model fused by the mixing matrix. In other words, while the average of $\x^i_t$ is not preserved due to directed communication, the average of the de-biased quantities $\z^i_t$ will be preserved \cite{nedic2014distributed}.

In addition to addressing challenges that arise from directed communication, the proposed algorithm deals with two sources of variance that hamper the convergence: a local variance that stems from noise in the local stochastic gradients, and a global variance that stems from the heterogeneity of the nodes' data. To address the former, we rely on momentum-based variance-reduction, while to tackle the latter we deploy gradient tracking.

%Specifically, the model $\z^i_t$ is used  as the input to query the stochastic first-order oracle for the gradient estimates. 
Let $\nabla f_i(\mathbf{z}^i_{t+1}, \mathbf{\xi}^i_{t})$ and $\nabla f_i(\mathbf{z}^i_{t}, \mathbf{\xi}^i_{t})$ denote stochastic gradients obtained after querying the local stochastic first-order oracle with $\mathbf{z}^i_{t+1} $ and $\mathbf{z}^i_{t}$, respectively. The momentum-type update of gradient $\v^i_{t+1}$ is then found as
\begin{equation}
    \mathbf{v}^i_{t+1} =  \nabla f_i(\mathbf{z}^i_{t+1}, \mathbf{\xi}^i_{t}) + (1-\beta)(\mathbf{v}^i_{t} -\nabla f_i(\mathbf{z}^i_{t}, \mathbf{\xi}^i_{t} ) ),
    \label{eq:update_v}
\end{equation}
where $\beta$ denotes the momentum step size controlling the direction of the gradient adjustment term $\mathbf{v}^i_{t} -\nabla f_i(\mathbf{z}^i_{t}, \mathbf{\xi}^i_{t} ) $. This recursive estimator reduces the variance of the stochastic gradient estimates in both centralized and distributed optimization problems \cite{cutkosky2019momentum,sun2020improving}. 
%[Note that (\ref{eq:update_v}) can equivalently be written as a convex combination of the vanilla stochastic gradient and a SARAH-type gradient estimate \cite{cutkosky2019momentum}.] 
Finally, the estimate of the global gradient is found via gradient tracking as
\begin{equation}
    \mathbf{g}_{t+1}^i = \sum_{j=1}^n w_{ij}^{(t)}(\mathbf{g}_t^j + \mathbf{v}_{t+1}^j - \mathbf{v}_{t}^j ) ,
\end{equation}
where the gradient information from neighboring nodes is used to ensure convergence to the first-order stationary point of the global objective.

The above procedure is formalized as Algorithm~1 and in the remainder of the paper referred to as the Push-ASGD (\underline{Push} \underline{A}ccelerated \underline{S}tochastic \underline{G}radient \underline{D}escent) algorithm.

==> n_bib.tex <==

@manual{kaggle,
  title  = "The Stack Overflow Data",
  url    = "https://www.kaggle.com/stackoverflow/stackoverflow",
}
@article{
koloskova2019decentralizeda,
  title={Decentralized deep learning with arbitrary communication compression},
  author={Koloskova, Anastasia and Lin, Tao and Stich, Sebastian U and Jaggi, Martin},
  journal={arXiv preprint arXiv:1907.09356},
  year={2019}
}
@article{xin2021hybrid,
  title={A hybrid variance-reduced method for decentralized stochastic non-convex optimization},
  author={Xin, Ran and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:2102.06752},
  year={2021}
}
@inproceedings{chen2023accelerated,
  title={Accelerated Distributed Stochastic Non-Convex Optimization over Time-Varying Directed Networks},
  author={Chen, Yiyue and Hashemi, Abolfazl and Vikalo, Haris},
  booktitle={ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}
@article{yuan2020can,
  title={Can primal methods outperform primal-dual methods in decentralized dynamic optimization?},
  author={Yuan, Kun and Xu, Wei and Ling, Qing},
  journal={IEEE Transactions on Signal Processing},
  volume={68},
  pages={4466--4480},
  year={2020},
  publisher={IEEE}
}
@article{towfic2015stability,
  title={Stability and performance limits of adaptive primal-dual networks},
  author={Towfic, Zaid J and Sayed, Ali H},
  journal={IEEE Transactions on Signal Processing},
  volume={63},
  number={11},
  pages={2888--2903},
  year={2015},
  publisher={IEEE}
}
@article{chen2021decentralized,
  title={Communication-efficient algorithms for decentralized optimization over directed graphs},
  author={Chen, Yiyue and Hashemi, Abolfazl and Vikalo, Haris},
  journal={arXiv e-prints},
  pages={arXiv--2005},
  year={2020}
}
@article{hashemi2021benefits,
  title={On the Benefits of Multiple Gossip Steps in Communication-Constrained Decentralized Federated Learning},
  author={Acharya, Anish and Hashemi, Abolfazl and  Das, Rudrajit and Vikalo, Haris and Sanghavi, Sujay and Dhillon, Inderjit S},
  journal={IEEE Transactions on Parallel and Distributed Systems},
  year={2021},
  publisher={IEEE}
}
@article{antoniadis2011penalized,
  title={Penalized likelihood regression for generalized linear models with non-quadratic penalties},
  author={Antoniadis, Anestis and Gijbels, Ir{\`e}ne and Nikolova, Mila},
  journal={Annals of the Institute of Statistical Mathematics},
  volume={63},
  number={3},
  pages={585--615},
  year={2011},
  publisher={Springer}
}
@article{cutkosky2019momentum,
  title={Momentum-Based Variance Reduction in Non-Convex SGD},
  author={Cutkosky, Ashok and Orabona, Francesco},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@inproceedings{stich2018sparsified,
  title={Sparsified {SGD} with memory},
  author={Stich, Sebastian U and Cordonnier, Jean-Baptiste and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4447--4458},
  year={2018}
}
@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}
@inproceedings{assran2019stochastic,
  title={Stochastic gradient push for distributed deep learning},
  author={Assran, Mahmoud and Loizou, Nicolas and Ballas, Nicolas and Rabbat, Mike},
  booktitle={International Conference on Machine Learning},
  pages={344--353},
  year={2019},
  organization={PMLR}
}
@inproceedings{tang2018communication,
  title={Communication compression for decentralized training},
  author={Tang, Hanlin and Gan, Shaoduo and Zhang, Ce and Zhang, Tong and Liu, Ji},
  booktitle={Advances in Neural Information Processing Systems},
  pages={7652--7662},
  year={2018}
}
@article{benaych2019largest,
  title={Largest eigenvalues of sparse inhomogeneous Erd{\H{o}}s--R{\'e}nyi graphs},
  author={Benaych-Georges, Florent and Bordenave, Charles and Knowles, Antti and others},
  journal={The Annals of Probability},
  volume={47},
  number={3},
  pages={1653--1676},
  year={2019},
  publisher={Institute of Mathematical Statistics}
}
@inproceedings{koloskova2019decentralized,
  title={Decentralized Stochastic Optimization and Gossip Algorithms with Compressed Communication},
  author={Koloskova, Anastasia and Stich, Sebastian and Jaggi, Martin},
  booktitle={International Conference on Machine Learning},
  pages={3478--3487},
  year={2019}
}
@article{erdos1959random,
  title={On random graphs},
  author={Erd{\"o}s, Paul and R{\'e}nyi, Alfr{\'e}d and others},
  journal={Publicationes mathematicae},
  volume={6},
  number={26},
  pages={290--297},
  year={1959}
}
@article{nedic2017achieving,
  title={Achieving geometric convergence for distributed optimization over time-varying graphs},
  author={Nedic, Angelia and Olshevsky, Alex and Shi, Wei},
  journal={SIAM Journal on Optimization},
  volume={27},
  number={4},
  pages={2597--2633},
  year={2017},
  publisher={SIAM}
}
@inproceedings{kempe2003gossip,
  title={Gossip-based computation of aggregate information},
  author={Kempe, David and Dobra, Alin and Gehrke, Johannes},
  booktitle={44th Annual IEEE Symposium on Foundations of Computer Science, 2003. Proceedings.},
  pages={482--491},
  year={2003},
  organization={IEEE}
}

@article{nedic2014distributed,
  title={Distributed optimization over time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={60},
  number={3},
  pages={601--615},
  year={2014},
  publisher={IEEE}
}
@article{jadbabaie2003coordination,
  title={Coordination of groups of mobile autonomous agents using nearest neighbor rules},
  author={Jadbabaie, Ali and Lin, Jie and Morse, A Stephen},
  journal={IEEE Transactions on automatic control},
  volume={48},
  number={6},
  pages={988--1001},
  year={2003},
  publisher={IEEE}
}
@article{ren2005consensus,
  title={Consensus seeking in multiagent systems under dynamically changing interaction topologies},
  author={Ren, Wei and Beard, Randal W},
  journal={IEEE Transactions on automatic control},
  volume={50},
  number={5},
  pages={655--661},
  year={2005},
  publisher={IEEE}
}
@article{ren2007information,
  title={Information consensus in multivehicle cooperative control},
  author={Ren, Wei and Beard, Randal W and Atkins, Ella M},
  journal={IEEE Control systems magazine},
  volume={27},
  number={2},
  pages={71--82},
  year={2007},
  publisher={IEEE}
}
@inproceedings{mcmahan2017communication,
  title={Communication-Efficient Learning of Deep Networks from Decentralized Data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial Intelligence and Statistics},
  pages={1273--1282},
  year={2017}
}

@techreport{tsitsiklis1984problems,
  title={Problems in decentralized decision making and computation.},
  author={Tsitsiklis, John Nikolas},
  year={1984},
  institution={Massachusetts Inst of Tech Cambridge Lab for Information and Decision Systems}
}

@article{boyd2006randomized,
  title={Randomized gossip algorithms},
  author={Boyd, Stephen and Ghosh, Arpita and Prabhakar, Balaji and Shah, Devavrat},
  journal={IEEE transactions on information theory},
  volume={52},
  number={6},
  pages={2508--2530},
  year={2006},
  publisher={IEEE}
}

@article{xiao2004fast,
  title={Fast linear iterations for distributed averaging},
  author={Xiao, Lin and Boyd, Stephen},
  journal={Systems \& Control Letters},
  volume={53},
  number={1},
  pages={65--78},
  year={2004},
  publisher={Elsevier}
}

@article{nedic2009distributed,
  title={Distributed subgradient methods for multi-agent optimization},
  author={Nedic, Angelia and Ozdaglar, Asuman},
  journal={IEEE Transactions on Automatic Control},
  volume={54},
  number={1},
  pages={48--61},
  year={2009},
  publisher={IEEE}
}

@article{johansson2010randomized,
  title={A randomized incremental subgradient method for distributed optimization in networked systems},
  author={Johansson, Bj{\"o}rn and Rabi, Maben and Johansson, Mikael},
  journal={SIAM Journal on Optimization},
  volume={20},
  number={3},
  pages={1157--1170},
  year={2010},
  publisher={SIAM}
}

@inproceedings{wei2012distributed,
  title={Distributed alternating direction method of multipliers},
  author={Wei, Ermin and Ozdaglar, Asuman},
  booktitle={2012 IEEE 51st IEEE Conference on Decision and Control (CDC)},
  pages={5445--5450},
  year={2012},
  organization={IEEE}
}

@article{duchi2011dual,
  title={Dual averaging for distributed optimization: {C}onvergence analysis and network scaling},
  author={Duchi, John C and Agarwal, Alekh and Wainwright, Martin J},
  journal={IEEE Transactions on Automatic control},
  volume={57},
  number={3},
  pages={592--606},
  year={2011},
  publisher={IEEE}
}

@inproceedings{nedic2015decentralized,
  title={Decentralized online optimization with global objectives and local communication},
  author={Nedi{\'c}, Angelia and Lee, Soomin and Raginsky, Maxim},
  booktitle={2015 American Control Conference (ACC)},
  pages={4497--4503},
  year={2015},
  organization={IEEE}
}

@inproceedings{he2018cola,
  title={Cola: {D}ecentralized linear learning},
  author={He, Lie and Bian, An and Jaggi, Martin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={4536--4546},
  year={2018}
}

@article{xi2017distributed,
  title={On the distributed optimization over directed networks},
  author={Xi, Chenguang and Wu, Qiong and Khan, Usman A},
  journal={Neurocomputing},
  volume={267},
  pages={508--515},
  year={2017},
  publisher={Elsevier}
}
@inproceedings{cai2011average,
  title={Average consensus on general digraphs},
  author={Cai, Kai and Ishii, Hideaki},
  booktitle={2011 50th IEEE Conference on Decision and Control and European Control Conference},
  pages={1956--1961},
  year={2011},
  organization={IEEE}
}

@article{cai2014average,
  title={Average consensus on arbitrary strongly connected digraphs with time-varying topologies},
  author={Cai, Kai and Ishii, Hideaki},
  journal={IEEE Transactions on Automatic Control},
  volume={59},
  number={4},
  pages={1066--1071},
  year={2014},
  publisher={IEEE}
}

@inproceedings{zhang2017zipml,
  title={Zipml: {T}raining linear models with end-to-end low precision, and a little bit of deep learning},
  author={Zhang, Hantian and Li, Jerry and Kara, Kaan and Alistarh, Dan and Liu, Ji and Zhang, Ce},
  booktitle={Proceedings of the 34th International Conference on Machine Learning-Volume 70},
  pages={4035--4043},
  year={2017},
  organization={JMLR. org}
}

@inproceedings{wen2017terngrad,
  title={Terngrad: {T}ernary gradients to reduce communication in distributed deep learning},
  author={Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
  booktitle={Advances in neural information processing systems},
  pages={1509--1519},
  year={2017}
}

@article{cai2012average,
  title={Average consensus on general strongly connected digraphs},
  author={Cai, Kai and Ishii, Hideaki},
  journal={Automatica},
  volume={48},
  number={11},
  pages={2750--2761},
  year={2012},
  publisher={Elsevier}
}

@article{nedic2016stochastic,
  title={Stochastic gradient-push for strongly convex functions on time-varying directed graphs},
  author={Nedi{\'c}, Angelia and Olshevsky, Alex},
  journal={IEEE Transactions on Automatic Control},
  volume={61},
  number={12},
  pages={3936--3947},
  year={2016},
  publisher={IEEE}
}

@article{saadatniaki2018optimization,
  title={Optimization over time-varying directed graphs with row and column-stochastic matrices},
  author={Saadatniaki, Fakhteh and Xin, Ran and Khan, Usman A},
  journal={arXiv preprint arXiv:1810.07393},
  year={2018}
}

@article{xin2019distributed,
  title={Distributed stochastic optimization with gradient tracking over strongly-connected networks},
  author={Xin, Ran and Sahu, Anit Kumar and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:1903.07266},
  year={2019}
}

@article{schmidt2017minimizing,
  title={Minimizing finite sums with the stochastic average gradient},
  author={Schmidt, Mark and Le Roux, Nicolas and Bach, Francis},
  journal={Mathematical Programming},
  volume={162},
  number={1-2},
  pages={83--112},
  year={2017},
  publisher={Springer}
}

@inproceedings{johnson2013accelerating,
  title={Accelerating stochastic gradient descent using predictive variance reduction},
  author={Johnson, Rie and Zhang, Tong},
  booktitle={Advances in neural information processing systems},
  pages={315--323},
  year={2013}
}

@article{ram2010distributed,
  title={Distributed stochastic subgradient projection algorithms for convex optimization},
  author={Ram, S Sundhar and Nedi{\'c}, Angelia and Veeravalli, Venugopal V},
  journal={Journal of optimization theory and applications},
  volume={147},
  number={3},
  pages={516--545},
  year={2010},
  publisher={Springer}
}
@article{das2020faster,
  title={Faster non-convex federated learning via global and local momentum},
  author={Das, Rudrajit and Acharya, Anish and Hashemi, Abolfazl and Sanghavi, Sujay and Dhillon, Inderjit S and Topcu, Ufuk},
  journal={arXiv preprint arXiv:2012.04061},
  year={2020}
}

@article{xin2019variance,
  title={Variance-reduced decentralized stochastic optimization with accelerated convergence},
  author={Xin, Ran and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:1912.04230},
  year={2019}
}

@inproceedings{li2020communication,
  title={Communication-efficient distributed optimization in networks with gradient tracking and variance reduction},
  author={Li, Boyue and Cen, Shicong and Chen, Yuxin and Chi, Yuejie},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={1662--1672},
  year={2020},
  organization={PMLR}
}

@article{qu2017harnessing,
  title={Harnessing smoothness to accelerate distributed optimization},
  author={Qu, Guannan and Li, Na},
  journal={IEEE Transactions on Control of Network Systems},
  volume={5},
  number={3},
  pages={1245--1260},
  year={2017},
  publisher={IEEE}
}

@inproceedings{gharesifard2010does,
  title={When does a digraph admit a doubly stochastic adjacency matrix?},
  author={Gharesifard, Bahman and Cort{\'e}s, Jorge},
  booktitle={Proceedings of the 2010 American Control Conference},
  pages={2440--2445},
  year={2010},
  organization={IEEE}
}

@article{qureshi2021push,
  title={Push-SAGA: A decentralized stochastic algorithm with variance reduction over directed graphs},
  author={Qureshi, Muhammad I and Xin, Ran and Kar, Soummya and Khan, Usman A},
  journal={IEEE Control Systems Letters},
  year={2021},
  publisher={IEEE}
}

@article{kar2012distributed,
  title={Distributed parameter estimation in sensor networks: Nonlinear observation models and imperfect communication},
  author={Kar, Soummya and Moura, Jos{\'e} MF and Ramanan, Kavita},
  journal={IEEE Transactions on Information Theory},
  volume={58},
  number={6},
  pages={3575--3605},
  year={2012},
  publisher={IEEE}
}

@article{lian2017can,
  title={Can decentralized algorithms outperform centralized algorithms? a case study for decentralized parallel stochastic gradient descent},
  author={Lian, Xiangru and Zhang, Ce and Zhang, Huan and Hsieh, Cho-Jui and Zhang, Wei and Liu, Ji},
  journal={arXiv preprint arXiv:1705.09056},
  year={2017}
}

@article{lecun1989backpropagation,
  title={Backpropagation applied to handwritten zip code recognition},
  author={LeCun, Yann and Boser, Bernhard and Denker, John S and Henderson, Donnie and Howard, Richard E and Hubbard, Wayne and Jackel, Lawrence D},
  journal={Neural computation},
  volume={1},
  number={4},
  pages={541--551},
  year={1989},
  publisher={MIT Press}
}

@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{xin2020decentralized,
  title={Decentralized stochastic optimization and machine learning: A unified variance-reduction framework for robust performance and fast convergence},
  author={Xin, Ran and Kar, Soummya and Khan, Usman A},
  journal={IEEE Signal Processing Magazine},
  volume={37},
  number={3},
  pages={102--113},
  year={2020},
  publisher={IEEE}
}

@inproceedings{xu2015augmented,
  title={Augmented distributed gradient methods for multi-agent optimization under uncoordinated constant stepsizes},
  author={Xu, Jinming and Zhu, Shanying and Soh, Yeng Chai and Xie, Lihua},
  booktitle={2015 54th IEEE Conference on Decision and Control (CDC)},
  pages={2055--2060},
  year={2015},
  organization={IEEE}
}

@inproceedings{pu2018distributed,
  title={A distributed stochastic gradient tracking method},
  author={Pu, Shi and Nedi{\'c}, Angelia},
  booktitle={2018 IEEE Conference on Decision and Control (CDC)},
  pages={963--968},
  year={2018},
  organization={IEEE}
}

@article{alghunaim2020decentralized,
  title={Decentralized proximal gradient algorithms with linear convergence rates},
  author={Alghunaim, Sulaiman A and Ryu, Ernest K and Yuan, Kun and Sayed, Ali H},
  journal={IEEE Transactions on Automatic Control},
  volume={66},
  number={6},
  pages={2787--2794},
  year={2020},
  publisher={IEEE}
}

@article{fang2018spider,
  title={Spider: Near-optimal non-convex optimization via stochastic path integrated differential estimator},
  author={Fang, Cong and Li, Chris Junchi and Lin, Zhouchen and Zhang, Tong},
  journal={arXiv preprint arXiv:1807.01695},
  year={2018}
}

@article{pham2020proxsarah,
  title={ProxSARAH: An Efficient Algorithmic Framework for Stochastic Composite Nonconvex Optimization.},
  author={Pham, Nhan H and Nguyen, Lam M and Phan, Dzung T and Tran-Dinh, Quoc},
  journal={J. Mach. Learn. Res.},
  volume={21},
  pages={110--1},
  year={2020}
}

@article{chen2021communication,
  title={Communication-Efficient Variance-Reduced Decentralized Stochastic Optimization over Time-Varying Directed Graphs},
  author={Chen, Yiyue and Hashemi, Abolfazl and Vikalo, Haris},
  journal={IEEE Transactions on Automatic Control},
  year={2021}
}
@article{arjevani2019lower,
  title={Lower bounds for non-convex stochastic optimization},
  author={Arjevani, Yossi and Carmon, Yair and Duchi, John C and Foster, Dylan J and Srebro, Nathan and Woodworth, Blake},
  journal={arXiv preprint arXiv:1912.02365},
  year={2019}
}
@incollection{bottou2010large,
  title={Large-scale machine learning with stochastic gradient descent},
  author={Bottou, L{\'e}on},
  booktitle={Proceedings of COMPSTAT'2010},
  pages={177--186},
  year={2010},
  publisher={Springer}
}
@inproceedings{maas2011learning,
  title={Learning word vectors for sentiment analysis},
  author={Maas, Andrew and Daly, Raymond E and Pham, Peter T and Huang, Dan and Ng, Andrew Y and Potts, Christopher},
  booktitle={Proceedings of the 49th annual meeting of the association for computational linguistics: Human language technologies},
  pages={142--150},
  year={2011}
}
@inproceedings{sun2020improving,
  title={Improving the sample and communication complexity for decentralized non-convex optimization: Joint gradient estimation and tracking},
  author={Sun, Haoran and Lu, Songtao and Hong, Mingyi},
  booktitle={International Conference on Machine Learning},
  pages={9217--9228},
  year={2020},
  organization={PMLR}
}
@article{krizhevsky2012imagenet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={25},
  pages={1097--1105},
  year={2012}
}
@inproceedings{pan2020d,
  title={D-SPIDER-SFO: A Decentralized Optimization Algorithm with Faster Convergence Rate for Nonconvex Problems},
  author={Pan, Taoxing and Liu, Jun and Wang, Jie},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  number={02},
  pages={1619--1626},
  year={2020}
}

@inproceedings{karimi2016linear,
  title={Linear convergence of gradient and proximal-gradient methods under the polyak-{\l}ojasiewicz condition},
  author={Karimi, Hamed and Nutini, Julie and Schmidt, Mark},
  booktitle={Joint European conference on machine learning and knowledge discovery in databases},
  pages={795--811},
  year={2016},
  organization={Springer}
}
@article{nedich2022ab,
  title={AB/Push-Pull Method for Distributed Optimization in Time-Varying Directed Networks},
  author={Nedich, Angelia and Nguyen, Duong Thuy Anh and Nguyen, Duong Tung},
  journal={arXiv preprint arXiv:2209.06974},
  year={2022}
}
@article{xin2020near,
  title={A near-optimal stochastic gradient method for decentralized non-convex finite-sum optimization},
  author={Xin, Ran and Khan, Usman A and Kar, Soummya},
  journal={arXiv preprint arXiv:2008.07428},
  year={2020}
}
@article{qureshi2020s,
  title={S-ADDOPT: Decentralized stochastic first-order optimization over directed graphs},
  author={Qureshi, Muhammad I and Xin, Ran and Kar, Soummya and Khan, Usman A},
  journal={IEEE Control Systems Letters},
  volume={5},
  number={3},
  pages={953--958},
  year={2020},
  publisher={IEEE}
}
@article{nguyen2023accelerated,
  title={Accelerated $ AB $/Push-Pull Methods for Distributed Optimization over Time-Varying Directed Networks},
  author={Nguyen, Duong Thuy Anh and Nguyen, Duong Tung and Nedich, Angelia},
  journal={arXiv preprint arXiv:2302.01214},
  year={2023}
}
